Space-time goal-oriented reduced basis approximation for linear wave equation

In this paper, we study numerically the linear damped second-order hyperbolic partial differential equation (PDE) with affine parameter dependence using a goal-oriented approach by finite element (FE) and reduced basis (RB) methods. The main contribution of this paper is the "goal-oriented" proper orthogonal decomposition (POD)-Greedy sampling procedure within the RB approximation context. First, we introduce the RB recipe: Galerkin projection onto a space $Y_N$ spanned by solutions of the governing PDE at $N$ selected points in parameter space. This set of $N$ parameter points is constructed by the standard POD-Greedy sampling procedure already developed. Second, based on the affine parameter dependence, we make use of the offline-online computational procedures: in the offline stage, we generate the RB space; in the online stage, given a new parameter value, we calculate rapidly and accurately the space-time RB output of interest and its associated asymptotic error. The proposed goal-oriented POD-Greedy sampling procedure can now be implemented and will look for the parameter points such that it minimizes this (asymptotic) output error rather than the solution error (or, error indicator which is the dual norm of residual) as in the standard POD-Greedy procedure. Numerical results show that the new goal-oriented POD-Greedy sampling procedure improves significantly the accuracy of the space-time output computation in comparison with the standard POD-Greedy one. The method is thus ideally suited for repeated, rapid and reliable evaluation of input-output relationships within the space-time setting.

==> Makefile <==
.phony: all dvi pdf view bib hello-world tar

BASE = paper

all: dvi pdf hello-world tar

dvi: ${BASE}.dvi

${BASE}.dvi: ${BASE}.tex ${BASE}.bbl
	latex ${BASE}


${BASE}.bbl: ${BASE}.bib
	bibtex ${BASE}

pdf: ${BASE}.pdf

${BASE}.pdf:	${BASE}.tex ${BASE}.bbl	
	pdflatex ${BASE}


view:	${BASE}.dvi
	xdvi ${BASE}&

bib: ${BASE}.bbl

hello-world: hello-world.dvi

hello-world.dvi:
	latex hello-world

tar: learn.tar

TARSOURCE = ${BASE}.tex ${BASE}.pdf ${BASE}.bib \
	    doodle.eps doodle.pdf hello-world.tex Makefile 

learn.tar: ${TARSOURCE}
	tar cf learn.tar ${TARSOURCE}

